Experimental evaluation of architectural software performance design patterns in microservices

Microservice architectures and design patterns enhance the development of large-scale applications by promoting flexibility. Industrial practitioners perceive the importance of applying architectural patterns but they struggle to quantify their impact on system quality requirements. Our research aims to quantify the effect of design patterns on system performance metrics, e.g., service latency and resource utilization, even more so when the patterns operate in real-world environments subject to heterogeneous workloads. We built a cloud infrastructure to host a well-established benchmark system that represents our test bed, complemented by the implementation of three design patterns: Gateway Aggregation, Gateway Offloading, Pipe and Filters. Real performance measurements are collected and compared with model-based predictions that we derived as part of our previous research, thus further consolidating the actual impact of these patterns. Our results demonstrate that, despite the difficulty to parameterize our benchmark system, model-based predictions are in line with real experimentation, since the performance behaviors of patterns, e.g., bottleneck switches, are mostly preserved. In summary, this is the first work that experimentally demonstrates the performance behavior of microservices-based architectural patterns. Results highlight the complexity of evaluating the performance of design patterns and emphasize the need for complementing theoretical models with empirical data.

==> Biography.tex <==

Willem Meijer is a PhD student at Linköping University, Sweden, focusing on software quality and bug detection in machine learning software. Previously, he graduated cum laude with an MSc in Software Engineering and Distributed Systems at the University of Groningen, The Netherlands, where he wrote his master's thesis on pull-based software engineering in software ecosystems, and participated in research related to architectural knowledge management. After graduating, he joined the Gran Sasso Science Institute (GSSI), Italy, as a research intern to study performance modeling in microservice architectures. His research interests include, among others, software quality and maintainability, software architecture, knowledge management, mining software repositories, and model-driven software engineering.

Catia Trubiani is Associate Professor at the Gran Sasso Science Institute (GSSI), Italy. Her research interests include quality-based modeling and analysis of interacting heterogeneous distributed systems, feedback strategies on software architectures, more recently applied to cyber-physical systems. Catia is leading and collaborating with diverse teams working on software quality projects, while considering ethics-based concerns. Her research contributed to the GSSI Department of Excellence obtaining more than 7M Euros in additional funding from the Italian Ministry of University and Research. Besides her academic role, Catia holds the position of coordinating the GSSI committee for equal opportunities, wellbeing of the personnel, and against discrimination.  


Aldeida Aleti is a Professor at Monash University, specializing in the intersection of AI and software engineering. Her research focuses on developing AI methods that automate various software development tasks, including software design and testing. With her expertise, Aldeida has led and contributed to multiple teams working on AI and software engineering projects, amounting to a cumulative value exceeding \$10M. She takes pride and joy in mentoring and advising over 16 PhD students and 5 research fellows, contributing to their academic and professional growth. In addition to her academic role, Aldeida holds the position of Associate Dean for Engagement and Impact in the Faculty of IT at Monash University. 
